RESMatch: Referring Expression Segmentation in a Semi-Supervised Manner

Referring expression segmentation (RES), a task that involves localizing specific instance-level objects based on free-form linguistic descriptions, has emerged as a crucial frontier in human-AI interaction. It demands an intricate understanding of both visual and textual contexts and often requires extensive training data. This paper introduces RESMatch, the first semi-supervised learning (SSL) approach for RES, aimed at reducing reliance on exhaustive data annotation. Extensive validation on multiple RES datasets demonstrates that RESMatch significantly outperforms baseline approaches, establishing a new state-of-the-art. Although existing SSL techniques are effective in image segmentation, we find that they fall short in RES. Facing the challenges including the comprehension of free-form linguistic descriptions and the variability in object attributes, RESMatch introduces a trifecta of adaptations: revised strong perturbation, text augmentation, and adjustments for pseudo-label quality and strong-weak supervision. This pioneering work lays the groundwork for future research in semi-supervised learning for referring expression segmentation.

==> author-kit-CVPR2024-v2/0_abstract.tex <==
\begin{abstract}
Referring expression segmentation (RES), a task that involves localizing specific instance-level objects based on free-form linguistic descriptions, has emerged as a crucial frontier in human-AI interaction. It demands an intricate understanding of both visual and textual contexts and often requires extensive training data. This paper introduces RESMatch, the first semi-supervised learning (SSL) approach for RES, aimed at reducing reliance on exhaustive data annotation. Extensive validation on multiple RES datasets demonstrates that RESMatch significantly outperforms baseline approaches, establishing a new state-of-the-art. Although existing SSL techniques are effective in image segmentation, we find that they fall short in RES. Facing the challenges including the comprehension of free-form linguistic descriptions and the variability in object attributes, RESMatch introduces a trifecta of adaptations: revised strong perturbation, text augmentation, and adjustments for pseudo-label quality and strong-weak supervision. This pioneering work lays the groundwork for future research in semi-supervised learning for referring expression segmentation.
\end{abstract}

==> author-kit-CVPR2024-v2/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Referring expression segmentation (RES) has emerged as an intriguing frontier in human-AI interaction \cite{Hu23, Kim23, wang2019reinforced}. Given an image and a textual description like ``the woman in the red dress", referring segmentation models delineate the precise pixels corresponding to the referred entity. Compared to classical segmentation tasks \cite{ronneberger2015u, chen2017deeplab, chen2018encoder} that categorize predefined labels, referring segmentation could enable the natural directing of autonomous systems and unlock more intuitive modes of instruction for AI agents. 
\begin{figure}[t]
  \centering
   \includegraphics[width=8.5cm]{author-kit-CVPR2024-v2/sec/head.png}  % 替换为你的图片文件名
  \caption{\textbf{This work proposes RESMatch, the first Semi-Supervised Learning (SSL) pipeline for referring expression segmentation.} We find that existing SSL approaches for image segmentation with added text encoder (FixMatch in this figure) cannot be directly applied to RES. They usually misunderstood regions defined by text (\emph{e.g.}, misidentification of regions, excessive or insufficient recognition).}
  \label{fig:head}
\end{figure}
Despite the promising applications, referring segmentation is a non-trivial task. Unlike semantic segmentation, which assigns categorical labels, RES requires localizing specific instance-level objects based on free-form linguistic descriptions. This introduces additional challenges in contextual reasoning and grounding language to elements in an image. The text query may describe attributes, relationships to other entities, or background scene details to identify the target object. As such, referring to segmentation demands finer-grained understanding compared to coarse semantic segmentation. To achieve this level of image understanding, a large amount of training data is typically required. As always, the more data used, the more likely it is to obtain better results. In addition, as referring expressions can use arbitrary vocabulary and compositional language constructs beyond a fixed vocabulary, the space of possible referring expressions for an object is vast. This makes data annotation more expensive compared to categorical labeling.



Meanwhile, as demonstrated by research in the realm of conventional image segmentation, annotating pixel-level semantic labels is an arduous, costly, and time-consuming endeavor. The challenges escalate further when confronted with the RES task. \textit{Can we find alternative avenues that reduce the reliance on massive amounts of training data? }

This work aims to tackle the problem \textbf{by proposing the first semi-supervised learning (SSL) approach for referring expression segmentation}. SSL \cite{liu2021unbiased, chen2021semi} is a powerful paradigm that involves acquiring new concepts from a limited number of annotated examples and many unannotated samples. As far as we know, SSL has not been exploited for referring expression segmentation, despite wide popularity mostly on image detection \cite{sohn2020simple, xu2021end}, some on image segmentation \cite{wang2022semi, yuan2022simple}, Existing SSL approaches have evolved from GANs-based adversarial training \cite{mittal2019semi,goodfellow2014generative,souly2017semi} into the widely adopted consistency regularization \cite{zou2020pseudoseg,chen2021semi,french2019semi,ouali2020semi,hu2021semi, huo2021atso,wang2022semi} and self-training \cite{yuan2022simple,he2021re,yang2022st++,guan2022unbiased} pipeline. Particularly, FixMatch \cite{sohn2020fixmatch} and Flexmatch \cite{zhang2021flexmatch} have gained increasing popularity with the competitive result by combining consistency regularization and pseudo labeling. These approaches employ a weak-to-strong supervision with teacher and student networks. A model's prediction for a weakly perturbed unlabeled input supervises its strongly perturbed counterpart. The paradigm has been demonstrated effective in semi-supervised image segmentation, but \textit{can they directly applied to referring expression segmentation?}

Unfortunately, the answer is \textit{No}. We try existing state-of-the-art SSL approaches with an added text encoder. The model often misunderstands the regions specified by the input text, segmenting either partially unwanted regions or missing some desired regions. (Cases shown in Fig. \ref{fig:head}, with more details in the experiment section). However, upon further examination, we propose that incorporating three modified design choices could dramatically alleviate these issues. The following highlights our key designs:

\noindent{\textbf{Design 1: Revisiting the Strong Perturbation}} is required, since we find not every strong perturbation approach fits the referring expression segmentation task as they may change the locations, colors, and relationships of other entities in an image, but these information are critical and may be involved in text descriptions.

\noindent{\textbf{Design 2: Applying Text Augmentation}} is needed, as referring expressions can use arbitrary vocabulary and structures. Given the limited availability of annotated samples, exposing the network to diverse expressions can help the model develop a stronger understanding of text and more robust abilities to connect text to imaged regions. 

\noindent{\textbf{Design 3: Pseudo-Label Quality and Strong-Weak Supervision Adjustment}} is introduced. We find that, unlike categorical semantic segmentation tasks that have multiple annotated regions in an image, RES often have only coarse labeling, leading to unsatisfactory pseudo-label quality. Adjustment in pseudo labels and applying the pseudo labeling in strong-weak supervision is required to prevent the model from being misled by unreliable pseudo-labels. 

By incorporating these three designs, we present RESMatch, the first semi-supervised learning approach for referring expression segmentation. We conducted extensive validations on multiple widely used datasets for RES and found that our approach achieves state-of-the-art (SOTA) performance, surpassing existing out-of-the-shelf SSL approaches by a significant margin. We believe that our work can serve as a valuable starting point for future research in the field of referring expression segmentation.



==> author-kit-CVPR2024-v2/2_formatting.tex <==
% \section{Related work}
% \textbf{Referring image segmentation.} Referring Expression Segmentation (RES) stands out as a crucial multi-modal task, integrating both language and image information. In the context of a provided image and a natural language expression, RES aims to produce a corresponding segmentation mask \cite{Hu16}. This task holds significant potential across various applications, including but not limited to video production and human-machine interaction.

% Several fully-supervised methods have been developed for this task, with earlier works primarily focusing on concatenating extracted multi-modal features \cite{Liu17, Li18}. As deep learning technology has advanced, more recent efforts have centered around the fusion of features extracted from different modalities \cite{Ye19,Chen19,Luo20,Hu20,Jing21,Ding21,Feng21,Kim22,Yang22,Wang22,Wu22}, as well as the optimization of performance for the essence of the RES problem \cite{Liu23, Xu23}. Recently, there has been a shift towards proposing more realistic and general models to address task-related RES problems \cite{Wu23,Yu23,Xu23b,Tang23,Liu23b,Lee23,Kim23,Liu23c,Hu23}. These advancements open up possibilities for practical applications in various projects.

% Fully supervised RES methods exhibit strong performance, however, they demand dense annotations for target masks and detailed expressions describing the target object. To tackle this challenge, we introduce a novel baseline for semi-supervised RES that relies on only a small amount of labeled data.

% \noindent\textbf{Semi-Supervised Learning.} In the realm of machine learning, Semi-Supervised Learning (SSL) methods offer a valuable approach by harnessing a limited set of labeled data alongside a wealth of unlabeled data, thereby mitigating the need for laborious annotation efforts. Notably, SSL has found widespread application in domains such as object detection \cite{liu2021unbiased, sohn2020simple, xu2021end} and semantic segmentation \cite{chen2021semi, wang2022semi, yuan2022simple}, showcasing its efficacy. The task of semantic segmentation demands a substantial number of intricate label annotations, so it is important to effectively apply semi-supervision to semantic segmentation.  Two prominent strategies in semi-supervised semantic segmentation are Pseudo-labeling \cite{hu2021simple, nassar2021labels, taherkhani2021selfsupervised, wang2022debiased, sun2023corrmatch, qiao2023fuzzy, zhao2023instance, fan2023conservative, ju2023cafs, chen2023semi, tian2023improving} and Consistency Regularization \cite{xie2019unsupervised, wang2021tripled, huang2022semi, yang2023revisiting, wang2023conflict, wu2023querying, zou2020pseudoseg}. Pseudo-label based methods typically involve selecting a set of predictions to generate pseudo-labels, which are then used to fine-tune the model. On the other hand, consistency regularization-based methods aim to utilize network predictions from weakly augmented inputs as supervision for predictions on strongly augmented inputs. Recent state-of-the-art (SOTA) semi-supervised segmentation methods \cite{yuan2022simple, zhong2021pixel, wang2023hunting, zhao2023augmentation} have ventured to combine both pseudo-labeling and consistency regularization or have focused on optimizing practical applications. These advancements emphasize the dynamic landscape and continuous refinement of semi-supervised learning techniques within the realm of semantic segmentation.

% Semi-supervised semantic segmentation in RES is similar to semantic segmentation, but RES only segments targets specified by text. Not only does it have the problem of foreground and background imbalance, but the addition of text also brings new challenges to semi-supervised segmentation. In this study, addressing the aforementioned issues, we pioneer the application of semi-supervised learning to RES, conducting a comprehensive exploration. Our proposed method, RESMatch, not only effectively tackles the challenges mentioned earlier but also addresses the intricacies of annotating complex and extensive datasets. This innovative approach not only enhances segmentation accuracy but also provides a practical solution to the challenges associated with annotating large and diverse datasets.

\section{Related work}
\textbf{Referring Expression Segmentation.} Referring expression segmentation (RES) is one of the most important multi-modal tasks, involving both language and image information. Unlike the conventional semantic segmentation task \cite{chen2017deeplab,zhu2023continual,zhu2021learning,zhu2023llafs,kirillov2023segment,chen2023sam}, the goal of RES is to generate a corresponding segmentation mask with the input of a natural language expression in the given image \cite{Hu16}. It has great potential in many applications, such as video production, and human-machine interaction.

There have been several fully-supervised methods for this task, prior works mainly focused on simply concatenating extracted multi-modal features \cite{Liu17, Li18}. With the development of deep learning technology, Most works focus on how to fuse two extracted features in different modalities 
\cite{Ye19,Chen19,Luo20,Hu20,Jing21,Ding21,Feng21,Kim22,Yang22,Wang22,Wu22} and performance optimization of the essence of RES problem \cite{Liu23, Xu23}. Recently, some work has proposed more realistic and general models to solve task-related RES problems \cite{Wu23,Yu23,Xu23b,Tang23,Liu23b,Lee23,Kim23,Liu23c,Hu23}, providing the possibility for practical application of projects.

Fully supervised RES methods show good performances, but they require dense annotations for target masks and comprehensive expressions describing the target object. To address this problem, we propose a new baseline for semi-supervised RES using only a small amount of labeled data.

\noindent\textbf{Semi-Supervised Learning.} Semi-supervised learning (SSL) methods leverage a few labeled data and abundant unlabeled data to reduce the dependency on laborious annotation. Recently, SSL has been widely used in object detection \cite{liu2021unbiased,sohn2020simple,xu2021end} and semantic segmentation \cite{chen2021semi,wang2022semi,yuan2022simple} and demonstrated its effectiveness. Semantic segmentation task requires a large number of complex label annotations, so it is important to effectively apply semi-supervision to semantic segmentation. Pseudo-label \cite{hu2021simple,nassar2021labels,taherkhani2021selfsupervised,wang2022debiased,sun2023corrmatch,qiao2023fuzzy,zhao2023instance,fan2023conservative,ju2023cafs,chen2023semi,tian2023improving} and consistency regularization \cite{xie2019unsupervised,wang2021tripled,huang2022semi,yang2023revisiting,wang2023conflict,wu2023querying,zou2020pseudoseg} are two effective strategies in semi-supervised semantic segmentation. Most pseudo-label based methods select a set of predictions to generate pseudo-labels to fine-tune the model while most of the consistency regularization-based methods aim at using the network predictions of the weakly augmented inputs as the supervision for those predictions of the strongly augmented inputs. More recently, SOTA semi-supervised segmentation methods \cite{yuan2022simple,zhong2021pixel,wang2023hunting,zhao2023augmentation} combine both two technologies together or focus on better application in practice. 

Semi-supervised semantic segmentation in RES is similar to semantic segmentation, but RES only segments targets specified by text. Not only does it have the problem of foreground and background imbalance, but the addition of text also brings new challenges to semi-supervised segmentation. In this work, In response to the above problems, we applied semi-supervision to RES for the first time conducted in-depth exploration, and proposed RESMatch, which not only effectively solved the above problems, but also solved complex and huge data annotation problems.

==> author-kit-CVPR2024-v2/3_finalcopy.tex <==

\section{Method}


%-------------------------------------------------------------------------
\subsection{Task Definition}
Performing the referring expression segmentation in a semi-supervised manner means the dataset contains the labeled set $D_x=\left\{\left(I_i^x, T_i^x\right), Y_i^x\right\}_{i=1}^{N^x}$ as well as an unlabeled set $D_u=\left\{\left(I_i^u, T_i^u\right)\right\}_{i=1}^{N^u}$, where $I$, $T$ and $Y$ denote the images, expressions and mask annotations, respectively. $N_x$ and $N_u$ denote the number of samples contained in $D_x$ and $D_u$. The training process aims to leverage both the $D_x$ and $D_u$ for accurately segmenting pixel-wise image regions based on text expressions.

\begin{figure*}[t]
  \centering
  % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}} % 注释掉这行
  \includegraphics[width=1.0\linewidth]{author-kit-CVPR2024-v2/sec/1.png}  % 替换为你的图片文件名
  \caption{\textbf{Illustration of Our Proposed RESMatch.} In RESMatch, labeled data $\{(I^x,T^x),Y^x\}$ is used to train the RES model $F$ by minimizing the supervised loss $L_{sup}$. Unlabeled data $(I^u,T^u)$, weakly augmented by $A^w(\cdot)$, is first fed into the model \textit{\^{F}} to obtain predictions $p^w$. The pseudo-label quality is based on the predicted confidence map, denoted as $s$. Based on the quality score, image strong augmentation $\phi$ is applied to the unlabeled data. Meanwhile, the semantic relevance filtering $\psi$ is applied with the strong text augmentation, denoted as $A^s(\cdot)$, The unsupervised loss $L_{unsup}$ is computed as the cross-entropy between $p^w$ and $p^s$, weighted by the quality of pseudo-labels $s$ to obtain predictions $p^s$ from the model $F$}
  \label{fig:pineline}
\end{figure*}

%Given a set of labeled data $D_s=\left\{\left(I_i^s, T_i^s\right), Y_i^s\right\}_{i=1}^{N^s}$ and unlabeled data $D_u=\left\{\left(I_i^u, T_i^u\right)\right\}_{i=1}^{N^u}$, the target of semi-supervised RES can be formulated as
%\begin{equation}
%\min \mathrm{L}\left(F ; D_s, D_u\right)
%\end{equation}

%where $L$ is the semi-supervised objective function. $\theta$ denotes the RES models $I$, $T$ and $Y$ denote the images, expressions and mask annotations, respectively. In practice, the numbers of labeled and unlabeled data meet $N_s \ll N_u$.

\subsection{RESMatch Network}
\subsubsection{Overview}
%How to effectively leverage the unlabeled data to enhance model performance is the key challenge for semi-supervised learning. FixMatch proposes a fundamental solution to address this problem based on a weak-to-strong consistency regularization mechanism. In this mechanism, predictions from weakly perturbed versions of unlabeled data act as supervisory signals for their strongly perturbed counterparts. Using the appropriate strong and weak augmentation methods is crucial to enhance the effectiveness of this mechanism, which should be carefully designed to ensure that: (1) the results after strong and weak augmentations are significant different so that overfitting can be avoided, and (2) the images after strong augmentation are not distorted too much so that they can still correspond to the same labels as the weakly augmented samples. Based on these results, 

%In this way, the overall optimization objective for the student model can be defined by:
Illustrated in Fig. \ref{fig:pineline}, the overall framework of RESMatch for semi-supervised RES follows the weak-to-strong consistency regularization framework, which is popularized by FixMatch \cite{sohn2020fixmatch}. During training, predictions from the weakly perturbed versions of unlabeled data serve as supervision signals for their strongly perturbed counterparts. The overall optimization objective for our model can be defined as:
%In this case, the overall optimization objective for the student is defined by
\begin{equation}
    \mathcal{L} = \lambda_x \mathcal{L}_{sup}+\lambda_{u}\mathcal{L}_{unsup},
\end{equation}

\noindent where $\lambda_x$ and $\lambda_u$ are hyperparameters used to respectively control the weights of the supervised loss and unsupervised loss. The supervised term $\mathcal{L}_{sup}$ is the cross-entropy loss between model predictions and ground truth labels. And the unsupervised loss $\mathcal{L}_{unsup}$ regularizes the prediction of the sample under strong perturbations to be the same as that under weak perturbations, which can be formulated as:
\begin{equation}
\mathcal{L}_{unsup} =\frac{1}{B_u} \sum \mathbbm{1}\left(\max \left(p^w\right) \geq \tau\right) \mathrm{H}\left(p^s, p^w\right),
\end{equation}
where $\mathbbm{1} (\cdot) $ is the indicator function, $B_u$ is the batch size for unlabeled data and $\tau$ is a pre-defined confidence threshold to filter noisy labels. $\rm{H}$ minimizes the entropy between two probability distributions:
\begin{equation}
    \begin{aligned}
    & p^w=\hat{F}\left(\textbf{\textit{A}}^w\left(I^u, T^u\right)\right) \\
    & p^s=F\left(\textbf{\textit{A}}^s\left(\textbf{\textit{A}}^w\left(I^u, T^u\right)\right)\right),
    \end{aligned}
\end{equation}
where the model produces pseudo labels on weakly perturbed images and texts and leverages strongly perturbed images and texts for model optimization. Following FixMatch \cite{sohn2020fixmatch}, we set \textit{\^{F}} the same as \textit{F}.

\subsubsection{Revisiting the Image Augmentation}
The augmentation strategy is critical for effectively utilizing labeled and unlabeled data in our weak-to-strong supervision framework, as demonstrated in prior works. However, we find that not all successful augmentation techniques for categorical image segmentation directly apply to our RES task. Our expressions often convey spatial relationships between objects (\emph{e.g.} ``woman on the right") and color information (\emph{e.g.} ``man with brown hair"). Thus, operations like CutMix and cropping that alter spatial layout are unsuitable, as they would disconnect the text expressions from corresponding image regions. Similarly, hue augmentation and pixel inversion disrupt color consistency. After analyzing standard techniques, we design custom augmentations that preserve spatial and color semantics to generate useful training signals from both labeled and unlabeled data. This allows full exploitation of our dataset in the semi-supervised setting. Eventually, the full list of our image augmentations is shown in Tab. \ref{table1}. Note that for some image augmentations, we change text expressions accordingly to preserve spatial and color semantics. For example, for augmentations like Random Horizontal Flip, we accordingly adapt text prompts defining spatial relationships (\emph{e.g.} flipping ``bags at left" to ``bags at right") to preserve semantics. For full analysis and more experimental results of testing different image augmentation strategies, please refer to the Supplementary Material. 

\begin{table}
  \centering
  \resizebox{\columnwidth}{!}{
 % \setlength{\tabcolsep}{30mm}{
    \begin{tabular}{@{}lp{8cm}@{}}
      \bottomrule[1pt]
      \multicolumn{2}{c}{\textbf{Weak} Augmentations} \\
      \hline
      Resize & Resize the image to the specified size. \\
      RandomHorizontalFlip & Horizontally flip the image with a probability of 0.5. \\
      \toprule
      \multicolumn{2}{c}{\textbf{Strong} intensity-based Augmentations} \\
      \hline
      Identity & Returns the original image. \\
      Autocontrast & Maximizes (normalize) the image contrast. \\
      Equalize & Equalize the image histogram.\\
      Gaussian blur & Blurs the image with a Gaussian kernel. \\
      Contrast & Adjusts the contrast of the image by [0.05, 0.95]. \\
      Sharpness & Adjusts the sharpness of the image by [0.05, 0.95].\\
      Color & Enhances the color balance of the image by [0.05, 0.95]. \\
      Brightness & Adjusts the brightness of the image by [0.05, 0.95].\\
      Posterize & Reduces each pixel to [4, 8] bits. \\
      \bottomrule[1pt]
    \end{tabular}}
  % }
  \caption{List of various image transformations in RESMatch.}
  \label{table1}
  
\end{table}

\subsubsection{Text Augmentation (TA)}
%Using the appropriate strong and weak augmentation methods is crucial to ensure the effectiveness of this mechanism, which should be carefully designed to ensure that: (1) the results after strong and weak augmentations are significant different so that overfitting can be avoided, and (2) the images after strong augmentation are not distorted too much so that they can still correspond to the same labels as the weakly augmented samples. Based on these results, 
As discussed earlier, existing SSL approaches designed for categorical image segmentation failed to perform well in our RES settings. One particular failure case is misunderstanding the arbitrary text expressions. We find image augmentations alone are insufficient - the text must also be distorted to improve understanding of descriptions. As mentioned, text augmentations are designed to match image changes, adapting spatial relations and color terms accordingly. Additionally, we employ NLP strategies to alter text expressions while retaining meaning, improving robustness to varied inputs. Our full multimodal-correlated text augmentation approach is outlined in Tab. \ref{table2}. By augmenting both modalities in a correlated manner, we enable the network to better comprehend arbitrary text-image relationships critical for reasoning about referential expressions. This allows properly utilizing unlabeled images with random text captions for SSL. 

%should necessitate simultaneous alterations to the color and positional words in its paired sentence.

%Data augmentation is widely used in deep learning to improve data efficiency and provide explicit regularization during model training in both computer vision (CV) and natural language processing (NLP). Applying existing data augmentation techniques to vision-language learning, however, is not straightforward. In an image-text pair, both the image and the text contain rich information that matches each other. Intuitively, we hope that their semantics still match after data augmentation. For example, consider an image with its paired sentence "a white dog playing in theright corner of the green lawn". Applying data augmentation methods such as cropping, color changing, and flipping to this image may require changing the color and positional words in its paired sentence at the same time.
%In order to preserve the semantic relationships, we have employed a set of straightforward, general-purpose NLP data augmentation techniques, as outlined in Table 2.

\begin{table}
  \centering
  \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lp{8cm}@{}}
     \bottomrule[1pt]
      \multicolumn{2}{c}{\textbf{Weak} Augmentations} \\
      \midrule
      Semantic-Preserving Change & Replace the position words in the sentence that match the image augmentation, \emph{e.g.}, ``left'' to ``right'', when the image of the corresponding sentence is flipped horizontally.
      \\
      \toprule
      \multicolumn{2}{c}{\textbf{Strong} Intensity-based Augmentations} \\
      \midrule
      Synonym Replacement(SR) & Replace n non-stop words in the sentence with random synonyms. \\
      Random Insertion(SI) & Insert synonyms of n random non-stop words into random positions in the sentence. \\
      Random Swap (RS) & Randomly choose two words in the sentence and swap their positions. \\
      Random Deletion (RD) & Randomly remove each word in the sentence with probability p.\\
      \bottomrule[1pt]
    \end{tabular}
  }
  \caption{List of text augmentations in RESMatch.}
  \label{table2}
\end{table}

To enhance diversity, we randomly generate 10 strongly-augmented texts per image using the methods in Tab. \ref{table2}. However, some texts may be semantically disrupted after the strong perturbation, affecting image-text pairing. To address this, we propose filtering out disrupted texts based on semantic intensity with the original weak text. Specifically, we extract BERT embeddings for each weak and strong text pair. Cosine similarity between embeddings measures semantic relevance:

\begin{align}
\theta_j=\frac{f_{s_j}^T \cdot f_w^T}{|f_{s_j}^T|\times| f_w^T |},
\end{align}

\noindent where $f_{s_j}^T$ and $f_w^T$ are strong and weak text embeddings, and $\theta_j$ is their semantic correlation. We do not greedily select most similar texts, as this causes an overfitted feature space. Instead, we remove those with $\theta_j<\lambda_t$ to retain enough perturbation while ensuring relevance. This allows generating diverse yet semantically meaningful weak-strong text pairs to improve regularization without disrupting original semantics.

\subsubsection{Model Adaptive Guidance (MAG)}
In the context of semi-supervised learning (SSL) in our referring expression segmentation (RES) settings, we face a more challenging scenario compared to categorical segmentation. This is primarily due to the scarcity of annotated semantic regions available for training, where typically only one annotated region per image is available for RES. Consequently, the performance of the generated pseudo masks is significantly impacted, resulting in the presence of noise and unreliability. Effectively addressing this limitation becomes a crucial challenge in SSL within RES settings.

Since generated pseudo masks can be noisy and unreliable, we introduce a mask-aware confidence score to assess each mask's quality for improved supervision. This score is the average confidence of all pixels in the mask above a threshold, as lower confidence pixels do not contribute to the loss. Formally, the score $s_i$ is calculated by:
\begin{equation}
s_i=\frac{\sum_{x, y}^{H, W} \mathbbm{1}\left(\max \left(p_{i, x, y}^w\right) \geq \tau\right) \cdot \max \left(p_{i, x, y}^w\right)}{\sum_{x, y}^{H, W} \mathbbm{1}\left(\max \left(p_{i, x, y}^w\right) \geq \tau\right)},
\end{equation}

\noindent the higher the mask-aware confidence score ($s_i$), the better the quality of the pseudo labels involved in training. We leverage this score to carefully adjust the augmentation strength during training. Specifically, we automatically decrease the augmentation strength if the pseudo mask has a lower $s_i$, and vice versa. This adaptive adjustment is motivated by the observation that a low-quality pseudo mask with a lower $s_i$ is often a consequence of overly strong augmentation, which can disrupt the data distribution.

By dynamically mixing the outputs of strongly-augmented and weakly-augmented samples, we achieve the augmentation adjustment. This ensures an appropriate enhancement strength that maintains semantic consistency while introducing necessary disturbance. The mixing process can be formulated as follows:
\begin{equation}
\textbf{\textit{A}}^s\left(I_i^u\right) \leftarrow s_i \textbf{\textit{A}}^s\left(I_i^u\right)+\left(1-s_i\right) \textbf{\textit{A}}^w\left(I_i^u\right).
\end{equation}
%where the distortion caused by the intensity-based strong augmentation is proportionally weakened by the corresponding weakly-augmented output.

In this way, instances with lower mask-aware confidence scores will not undergo significant perturbations during augmentation. This ensures that the model is not overly challenged by potentially out-of-distribution cases, allowing it to focus on learning from more reliable and representative instances.

Additionally, considering the varying learning difficulties of different instances, we leverage the obtained mask-aware confidence scores to design a self-adaptive unsupervised loss. This loss allows the model to learn from different unlabeled data in a tailored manner. The calculation of this loss is as follows:


\begin{equation}
    \begin{aligned}
    &{L}_{unsup}= \frac{1}{\left|{~B}_u\right|} \sum_{i=1}^{|{~B}_u \mid} \bigg[\frac{s_i}{H \times W} \\
    &\sum_{x, y}^{H, W} \mathbbm{1}\left(\max \left(p_{i, x, y}^w\right) \geq \tau\right) \mathrm{H}\left(\textbf{\textit{A}}^s\left(I^u_i, T^u_i\right), p^w_i\right)\bigg].
    \end{aligned}
\end{equation}


In this way, noise interference because of limited annotated sample of semantic regions is alleviated, thus significantly enhancing semi-supervised performance.


==> author-kit-CVPR2024-v2/4_experiments.tex <==
\section{Experiments}


%-------------------------------------------------------------------------
% \subsection{Experimental Setup}
% \label{sec:exp}

% \noindent \textbf{Dataset.}


% % \noindent \textbf{Backbone.}
% swin transforer


% \noindent \textbf{Implementation details.}
% baseline
\subsection{Datasets}

% We evaluate our method on three standard benchmark datasets, RefCOCO \cite{Yu_Poirson_Yang_Berg_Berg_2016}, RefCOCO+ \cite{Yu_Poirson_Yang_Berg_Berg_2016}, and RefCOCOg \cite{Nagaraja_Morariu_Davis_2016}. RefCOCO \& RefCOCO+ are obtained from MS-COCO   \cite{lin}. 19,994 images annotated with 142,209 referring expressions describing 50,000 objects are collected in the RefCOCO dataset, and 19,992 images associated with 141,564 referring expressions for 49,856 objects are collected in the RefCOCO+ dataset. There are four splits in RefCOCO and RefCOCO+, \emph{i.e.} train, val, testA and testB. The dataset RefCOCO has no restrictions on the referring expressions, while the dataset RefCOCO+ does not allow location-describing words in the expressions, \emph{e.g.} “topmost”. RefCOCOg is another well-known and widely recognized referring segmentation dataset. 26,711 images annotated with 104,506 referring expressions for 54,822 objects are used in the RefCOCOg datasets. Notably, we use the UMD split \cite{Nagaraja_Morariu_Davis_2016}, which contains three splits, \emph{i.e.}, training, validation and testing. In contrast to the two datasets described above, expressions in RefCOCOg (containing 8.4 words on average) are longer and complex. For semi-supervised learning, we randomly choose 0.1\%, 1\%, 5\%, and 10\% of the samples as labeled data, while the remaining data is allocated for unlabeled data.
We evaluate our method on three standard benchmark datasets: RefCOCO \cite{Yu_Poirson_Yang_Berg_Berg_2016}, RefCOCO+ \cite{Yu_Poirson_Yang_Berg_Berg_2016}, and RefCOCOg \cite{Nagaraja_Morariu_Davis_2016}. RefCOCO and RefCOCO+ are derived from MS-COCO \cite{lin}, consisting of 19,994 and 19,992 images, respectively. These images are annotated with 142,209 and 141,564 referring expressions, describing 50,000 and 49,856 objects in the RefCOCO and RefCOCO+ datasets. Both datasets have four splits: train, val, testA, and testB. RefCOCO allows arbitrary referring expressions, while RefCOCO+ excludes location-describing words, such as ``topmost", from the expressions. RefCOCOg, another well-known referring segmentation dataset, includes 26,711 images annotated with 104,506 referring expressions for 54,822 objects. We utilize the UMD split \cite{Nagaraja_Morariu_Davis_2016}, which comprises training, validation, and testing splits. In contrast to the former datasets, expressions in RefCOCOg are longer and more complex, averaging 8.4 words. 

In our experiment, for semi-supervised learning, we randomly select 0.1\%, 1\%, 5\%, and 10\% of the samples as labeled data, allocating the remaining data for unlabeled data.




\begin{table*}[h]
\begin{minipage}{\linewidth}
\resizebox{\textwidth}{!}{

\begin{tabular}{llcccllllllllllll}
\bottomrule[1pt]
\multicolumn{1}{c}{\multirow{2}{*}{Methods}} & \multicolumn{16}{c}{RefCOCO} \\ 
\cline{2-17} 
\multicolumn{1}{c}{}                         & \multicolumn{4}{c}{0.1\%} &  & \multicolumn{3}{c}{1\%} &  & \multicolumn{3}{c}{5\%} &  & \multicolumn{3}{c}{10\%} \\ 
\cline{1-5} \cline{7-9} \cline{11-13} \cline{15-17} 
                                             &  & val & testA & testB &  & val & testA & testB &  & val & testA & testB &  & val & testA & testB \\ 
\cline{3-5} \cline{7-9} \cline{11-13} \cline{15-17} 
Supervised                                   &  & 16.91 & 19.22 & 14.72 &  & 28.02 & 31.32 & 24.35 &  & 43.58 & 48.16 & 39.55 &  & 51.81 & 55.35 & 48.38 \\
Fixmatch \cite{sohn2020fixmatch}             &  & 18.82 & 21.05 & 16.74 &  & 33.89 & 38.46 & 30.17 &  & 49.18 & 52.81 & 44.30 &  & 54.55 & 57.91 & 51.92 \\
AugSeg \cite{zhao2023augmentation}            &  & 4.50  &  5.79 & 2.19  &  & 24.42 & 26.23 & 22.18 &  & 30.99 & 34.81 & 27.93 &  & 39.63 & 32.45 & 32.00 \\
CCVC \cite{wang2023conflict}                 &  & 15.22 & 16.32 & 15.16 &  & 28.14 & 32.23 & 24.29 &  & 46.62 & 49.92 & 42.37 &  & 53.13 & 56.48 & 49.51 \\
RESMatch                                     &  & \textbf{20.07} & \textbf{22.47} & \textbf{17.88} &  & \textbf{36.86} & \textbf{42.32} & \textbf{31.11} &  & \textbf{51.95} & \textbf{56.91} & \textbf{47.20} &  & \textbf{58.45} & \textbf{62.56} & \textbf{54.17} \\ 

\hline
\end{tabular}}

\vspace{0.4cm}
\resizebox{\textwidth}{!}{

\begin{tabular}{llcccllllllllllll}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Methods}} & \multicolumn{16}{c}{RefCOCO+} \\ 
\cline{2-17} 
\multicolumn{1}{c}{}                         & \multicolumn{4}{c}{0.1\%} &  & \multicolumn{3}{c}{1\%} &  & \multicolumn{3}{c}{5\%} &  & \multicolumn{3}{c}{10\%} \\ 
\cline{1-5} \cline{7-9} \cline{11-13} \cline{15-17} 
                                             &  & val & testA & testB &  & val & testA & testB &  & val & testA & testB &  & val & testA & testB \\ 
\cline{3-5} \cline{7-9} \cline{11-13} \cline{15-17} 
Supervised                                   &  & 17.44 & 19.28 & 15.73 &  & 25.62 & 28.53 & 22.56 &  & 36.05 & 39.87 & 30.71 &  & 40.49 & 44.48 & 34.50 \\
Fixmatch \cite{sohn2020fixmatch}                                     &  & 15.41 & 19.72 & 10.53 &  & 29.29 & 33.47 & 25.55 &  & 38.81 & 43.34 & 33.31 &  & 42.50 & 47.81 & 36.57 \\
AugSeg \cite{zhao2023augmentation}                                      &  & 5.69  & 10.13 & 0.63  &  & 22.43 & 25.35 & 19.49 &  & 33.23 & 36.68 & 28.22 &  & 35.07 & 38.48 & 31.17 \\
CCVC \cite{wang2023conflict}                                         &  & 14.59 & 15.30 & 14.77 &  & 29.12 & 32.44 & 25.31 &  & 37.30 & 41.37 & 32.20 &  & 41.38 & 45.24 & 35.76 \\
RESMatch                                     &  & \textbf{18.11} & \textbf{23.54} & \textbf{15.37} &  & \textbf{31.09} & \textbf{35.72} & \textbf{26.07} &  & \textbf{39.97} & \textbf{44.66} & \textbf{33.56} &  & \textbf{45.03} & \textbf{51.22} & \textbf{37.97} \\

\hline
\end{tabular}}

\vspace{0.4cm}
\setlength{\tabcolsep}{4mm}{
\resizebox{\textwidth}{!}{

\begin{tabular}{llcclcclcclcc}
\hline
\multicolumn{1}{c}{\multirow{2}{*}{Methods}} & \multicolumn{12}{c}{RefCOCOg} \\ 
\cline{3-13} 
\multicolumn{1}{c}{}                         &  & \multicolumn{2}{c}{0.1\%} &  & \multicolumn{2}{c}{1\%} &  & \multicolumn{2}{c}{5\%} &  & \multicolumn{2}{c}{10\%} \\ 
\cline{1-4} \cline{6-7} \cline{9-10} \cline{12-13} 
                                             &  & val-u & test-u &  & val-u & test-u &  & val-u & test-u &  & val-u & test-u \\ 
\cline{3-4} \cline{6-7} \cline{9-10} \cline{12-13} 
Supervised                                   &  & 16.97 & 17.14 &  & 26.23 & 26.92 &  & 34.58 & 36.50 &  & 40.43 & 41.58 \\
Fixmatch \cite{sohn2020fixmatch}              &  & 19.96 & \textbf{21.12} &  & 31.62 & \textbf{33.58} &  & 39.55 & 40.98 &  & \textbf{45.50} & 46.78 \\
AugSeg \cite{zhao2023augmentation}                                        &  & 1.05  & 0.94  &  & 24.07 & 24.71 &  & 34.08 & 35.31 &  & 37.02 & 38.28 \\
CCVC \cite{wang2023conflict}                                         &  & 11.58 & 11.70 &  & 29.35 & 30.57 &  & 37.76 & 39.23 &  & 42.50 & 43.49 \\
RESMatch                                     &  & \textbf{20.97} & 20.91 &  & \textbf{32.18} & 33.21 &  & \textbf{39.77} & \textbf{41.42} &  & 45.24 & \textbf{47.39}\\ 
\bottomrule[1pt] 
\end{tabular}}
}

\caption{\textbf{Comparison of RESMatch, our reproduced FixMatch and Supervised on RefCOCO, RefCOCO+, and RefCOCOg.} For all approaches, we use LAVT as the RES model. “Supervised” refers to the supervised training approach under various semi-supervised settings.}
\label{table3}

\end{minipage}
\end{table*}

\subsection{Evaluation Metrics}
As in previous works, we utilize widely-used metrics, overall Intersection over Union (oIoU), to assess the performance of our model. The overall IoU is computed as the ratio of the total intersection area to the total union area across all test samples. Each sample consists of a language expression paired with an image. This metric provides a comprehensive evaluation of the model's ability to accurately align language expressions with corresponding images.


\begin{table}
\renewcommand\arraystretch{1.25}
\setlength{\tabcolsep}{3.85mm}{
\begin{tabular}{p{2.9cm}llll}
\bottomrule[1pt]%\hline
Hyperparameter $\gamma$ & val   & testA  & testB  \\ \hline
0.5  & 58.11 & 62.13 & 53.25     \\
0.7  & \textbf{58.45} & \textbf{62.56} & \textbf{54.17} \\
0.9  & 57.51 & 60.70 & 53.74  \\ 
\bottomrule[1pt]%\hline
\end{tabular}}
\caption{Effect of the hyperparameter used in MAG.}
\label{tablexxx}
\end{table}

\begin{table}
\renewcommand\arraystretch{1.25}
\setlength{\tabcolsep}{3.85mm}{
\begin{tabular}{p{2.9cm}llll}
\bottomrule[1pt]%\hline
Method & val   & testA  & testB  \\ \hline
Supervised & 51.81 & 55.35 & 48.38 \\
RESMatch$_{1}$  & 59.19 & 63.10 & 53.90 \\
RESMatch$_{2}$ & 58.36     & 62.54     & 53.96     \\
RESMatch$_{3}$  & 58.87 & 63.68 & 53.96 \\ 
\bottomrule[1pt]%\hline
\end{tabular}}
\caption{Random partitioning on the RefCOCO dataset under the 10\% setting and 
results measured with oIoU.}
\label{table8}
\end{table}





\subsection{Implementation Details}
\begin{table}[h]
\renewcommand\arraystretch{1.25}
\begin{tabular}{p{4.2cm}llll}
\bottomrule[1pt]%\hline
Method                 & Ref   & Ref+  & Refg  \\ \hline
Supervised              & 43.58 & 36.05 & 34.58 \\
+ pseudo-label learning & 46.42     & 37.70     & 36.94     \\
+ semi-supervised opt.  & \textbf{51.95} & \textbf{39.97} & \textbf{39.77} \\ \bottomrule[1pt]%\hline
\end{tabular}
\caption{Ablation study of semi-supervised RES framework on 5\% RefCOCO, RefCOCO+ and RefCOCOg.}
\label{table4}
\end{table}

% We use LAVT \cite{Yang22} as our RES model, which utilizes swin-tiny \cite{swin}  pre-trained on ImageNet-22K \cite{imagenet} as the image encoder, BERT \cite{Devlin_Chang_Lee_Toutanova_2019} as the text encoder and randomly initialize the decoder. All models are trained by AdamW with a constant learning rate of 1e-5. The batch size is set to 2, which consists of 2 labeled and 2 unlabeled image-text pairs. The total training epoch are 40. Images are resized to 480×480 and data augmentation as shown in Table \ref{table1} and Table \ref{table2}. We set $\lambda_x$ = 5, $\lambda_u$ = 2, $\lambda_t$ = 0.8 and $\gamma$ = 0.7 in our experiments.




We adopt the LAVT model \cite{Yang22} as our RES model, utilizing swin-tiny \cite{swin} pre-trained on ImageNet-22K \cite{imagenet} for image encoding and BERT \cite{Devlin_Chang_Lee_Toutanova_2019} for text encoding. All models are trained using AdamW with a consistent learning rate of 1e-5. The batch size is set to 2. The total training epochs are set to 40. Image resizing is performed to 480×480, and data augmentation is applied according to the specifications outlined in Tab. \ref{table1} and Tab. \ref{table2}. In our experiments, we set the parameters $\lambda_x$ = 5, $\lambda_u$ = 2, $\lambda_t$ = 0.8, and $\gamma$ = 0.7. 

\begin{figure}[h]
  \centering
   \includegraphics[width=8.5cm]{author-kit-CVPR2024-v2/sec/2.png}  % 替换为你的图片文件名
  \caption{\textbf{Training curves of RESMatch and Supervised.} RESMatch can consistently improve performance throughout the whole training period more effectively than Supervised.}
  \label{fig:curves}
\end{figure}



\begin{table}[h]
\setlength{\tabcolsep}{3.85mm}{
\begin{tabular}{p{2.9cm}llll}
\bottomrule[1pt]%\hline
Method           & Ref       & Ref+      & Refg  \\ \hline
SemiBaseline     & 33.62     & 29.85     & 30.85     \\
+ TA             & 35.30     & 30.48     & 31.73 \\
+ MAG             & 35.17     & 29.86     & 31.38  \\
Ours             & \textbf{36.86} & \textbf{31.09} & \textbf{32.18} \\ \bottomrule[1pt]%\hline
\end{tabular}}
\caption{Ablation study of TA and MAG on 1\% RefCOCO val, RefCOCO+ val and RefCOCOg val.}
\label{table6}
\end{table}


\begin{figure*}[h]
  \centering
  \captionsetup[subfigure]{labelformat=empty} % 隐藏子图标签 (a), (b), ...

  \subfloat[\fontsize{11}{14}\selectfont(a) Comparison of 10\% Supervised and RESMatch on RefCOCO val.\\]{
  \setlength{\tabcolsep}{0.75mm}{
    \begin{tabular}{cccc}
  \multicolumn{1}{c}{Input} & \multicolumn{1}{c}{GT} & \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{RESMatch} \\
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp1-1.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp1-4.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp1-2.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp1-3.png} \\
    \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-1: person holding umbrella}} \\
 
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp3-1.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp3-4.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp3-2.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp3-3.png} \\
    \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-3: front bowl w/carrots in it}} \\

  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp5-1.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp5-4.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp5-2.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp5-3.png} \\
    \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-5: left guy}} \\
\end{tabular}}
    \hfill
    \setlength{\tabcolsep}{0.75mm}{
    \begin{tabular}{cccc}
      \multicolumn{1}{c}{Input} & \multicolumn{1}{c}{GT} & \multicolumn{1}{c}{Supervised} & \multicolumn{1}{c}{RESMatch} \\
      \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp2-1.png} &
      \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp2-4.png} &
      \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp2-2.png} &
      \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp2-3.png} \\
       \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-2: right chick}} \\
       
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp4-1.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp4-4.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp4-2.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp4-3.png} \\
   \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-4: bottom box left dude}} \\

  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp6-1.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp6-4.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp6-2.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp6-3.png} \\
    \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-6: left sandwich}} \\
    \end{tabular}
  }}
  
   \subfloat[\fontsize{11}{14}\selectfont(b) Comparison of 10\% Supervised and RESMatch on RefCOCO val.]{
   \setlength{\tabcolsep}{0.75mm}{
    \begin{tabular}{cccc}
  \multicolumn{1}{c}{Input} & \multicolumn{1}{c}{GT} & \multicolumn{1}{c}{w.o. TA} & \multicolumn{1}{c}{w.i. TA} \\
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp7-1.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp7-4.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp7-2.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp7-3.png} \\
    \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-7: black cat}} \\
 
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp8-1.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp8-4.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp8-2.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp8-3.png} \\
    \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-8: Pitcher}} \\

  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp9-1.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp9-4.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp9-2.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp9-3.png} \\
    \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-9: man not in purple}} \\
\end{tabular}}
    \hfill
    \setlength{\tabcolsep}{0.75mm}{
    \begin{tabular}{cccc}
      \multicolumn{1}{c}{Input} & \multicolumn{1}{c}{GT} & \multicolumn{1}{c}{w.o. MAG} & \multicolumn{1}{c}{w.i. MAG} \\
      \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp10-1.png} &
      \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp10-4.png} &
      \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp10-2.png} &
      \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp10-3.png} \\
       \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-10: luggage left side}} \\
       
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp11-1.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp11-4.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp11-2.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp11-3.png} \\
   \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-11: lady in purpl asian}} \\

  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp12-1.png} &
  \includegraphics[scale=0.11]{author-kit-CVPR2024-v2/sec/expfig/exp12-4.png} &
  \includegraphics[scale=0.108]{author-kit-CVPR2024-v2/sec/expfig/exp12-2.png} &
  \includegraphics[scale=0.108]{author-kit-CVPR2024-v2/sec/expfig/exp12-3.png} \\
    \multicolumn{4}{c}{\makebox[0pt]{\centering Exp-12: guy facing camera}} \\
    \end{tabular}}
  }
  \caption{\textbf{Visualizations of RESMatch and Supervised.} Sub-figure (a) shows the predictions of RESMatch are much better than Supervised. Sub-figure (b) indicates that both TA and MAG of RESMatch can obviously improve the quality of pseudo-labels. }
  \label{fig:vis1}
\end{figure*}

\subsection{Experimental Results}

% \subsubsection{Comparison with Baselines}

\subsubsection{Comparison with Fully Supervised Settings}
Experimental results have shown that additional data will benefit the performance of segmentation, which validate the effectiveness of our semi-supervised approach. 
Tab. \ref{table3} compares our semi-supervised RESMatch to fully-supervised LAVT baselines under varying labeling ratios (0.1\%, 1\%, 5\%, 10\%). RESMatch substantially outperforms the supervised models given the same number of annotations, demonstrating the benefits of leveraging unlabeled data. For example, with just 1\% labeled data, RESMatch improves over the supervised baseline by +8.84\% on RefCOCO val, +8.37\% on 5\% RefCOCO val, and +6.64\% on 10\% RefCOCO val. Remarkably, 10\% supervision achieves 87\% of the fully-supervised performance on RefCOCO testA. Gains are consistent across datasets (+5.47\% on 1\% RefCOCO+ val, +5.95\% on 1\% RefCOCOg val), evidencing the robustness of our approach. These results show that RESMatch successfully exploits unlabeled images via semi-supervised learning, overcoming limited annotations and approaching the performance ceiling of full supervision.

We specifically compare the training curves of RESMatch and Supervised in Fig. \ref{fig:curves} to reveal how the semi-supervised approach continues benefiting throughout training while supervised learning plateaus early on. This highlights the value of unlabeled data in improving model generalization and preventing overfitting to the limited labeled examples. The training dynamics further validate the effectiveness of RESMatch for low-resource referring expression segmentation.

\begin{figure*}[h]
  \centering
  \captionsetup[subfigure]{labelformat=empty} % 隐藏子图标签 (a), (b), ...
\subfloat[]{
    \setlength{\tabcolsep}{0.7mm}{
    \begin{tabular}{ccc}
  \multicolumn{1}{c}{Input}  & \multicolumn{1}{c}{GT} & \multicolumn{1}{c}{RESMatch} \\
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp13-1.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp13-3.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp13-2.png} \\
    \multicolumn{3}{c}{\makebox[0pt]{\centering \shortstack{Exp-13: left half of right \\ sandwich}}} \\
 
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp15-1.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp15-3.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp15-2.png} \\
    \multicolumn{3}{c}{\makebox[0pt]{\centering Exp-15: cather}} \\

\includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp17-1.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp17-3.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp17-2.png} \\
    \multicolumn{3}{c}{\makebox[0pt]{\centering Exp-17: the mans hair on right}} \\
\end{tabular}}
    \hfill
    \setlength{\tabcolsep}{0.7mm}{
    \begin{tabular}{ccc}
  \multicolumn{1}{c}{Input}  & \multicolumn{1}{c}{GT} & \multicolumn{1}{c}{RESMatch} \\
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp14-1.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp14-3.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp14-2.png} \\
    \multicolumn{3}{c}{\makebox[0pt]{\centering \shortstack{Exp-14: man in right front with blue \\ tie next to older woman}}} \\

  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp18-1.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp18-3.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp18-2.png} \\
    \multicolumn{3}{c}{\makebox[0pt]{\centering Exp-16: 33}} \\

\includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp16-1.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp16-3.png} &
  \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp16-2.png} \\
    \multicolumn{3}{c}{\makebox[0pt]{\centering Exp-18: item on right}} \\
\end{tabular}}
  }
  \vspace{-15pt} % 根据需要调整垂直间距
    \caption{\textbf{Failure cases of RESMatch.} RESMatch still fails in some hard examples. Such as abstract expressions and the ambiguity of text or images.}
  \label{fig:vis2}
\end{figure*}



\subsubsection{Ablation Study}


\noindent
\textbf{The impact of the semi-supervised framework.}  We conducted a series of experiments, as detailed in Tab. \ref{table4} and Tab. \ref{table3}, to assess the effectiveness of our semi-supervised approach. In Tab. \ref{table4}, we initially analyze the impact of the semi-supervised RES framework in RESMatch under the 5\% labeled data setting. The results indicate that pseudo-label learning contributes significantly to performance improvement across all three RES datasets, such as a notable +2.48\% on 5\% RefCOCO validation. Moreover, with the integration of semi-supervised optimization, such as strong-weak augmentations, the performance on 5\% RefCOCO improves from 46.42 to 51.95. These gains underscore the importance of addressing challenges related to suboptimal pseudo-labels, a concern alleviated through our semi-supervised optimization strategies.




In Tab. \ref{table3}, we compare our reproduced method with existing state-of-the-art SSL approaches on the RefCOCO dataset. The results clearly demonstrate that RESMatch has achieved noteworthy advancements, outperforming the competition.



\noindent
\textbf{The impact of TA and MAG.} In Tab. \ref{table6}, we analyze the effectiveness of TA and MAG in RESMatch. The results indicate that both design elements contribute to performance improvement. Notably, TA demonstrates more substantial gains than MAG, with an increase of +1.68\% on 1\% RefCOCO validation. Furthermore, the combination of TA with MAG leads to additional enhancements, elevating RESMatch's performance from 35.30 to 36.86 on 1\% RefCOCO validation. These findings robustly validate the effectiveness of TA.

\subsubsection{Qualitative analysis}

% To gain deeper insights into RESMatch, we perform comprehensive visualizations as shown in Fig. \ref{fig:vis1}. In Fig. \ref{fig:vis1} (a), we note that RESMatch's predictions exhibit more accurate target localization, as seen in examples like Exp-1 and Exp-2, more complete target recognition, illustrated by examples such as Exp-3 and Exp-4, and more precise boundary contour recognition, demonstrated in examples like Exp-5 and Exp-6.



% In Fig. \ref{fig:vis1} (b), we additionally compare the pseudo-labels with and without STE and MAG. These visualizations clearly show that both designs significantly enhance the quality of pseudo-labels.


%  We also visualize the cases of failure in Fig. \ref{fig:vis2}. We observe that RESMatch tends to struggle when dealing with highly abstract expressions, such as in Exp-13 and Exp-14, where multiple directional terms appear within the expression. Additionally, failures occur in instances like Exp-15 and Exp-16, where there is ambiguity in the text due to spelling errors and incomplete expressions. Moreover, ambiguity in the image contributes to failures, as seen in Exp-17 and Exp-18, where it becomes challenging to precisely distinguish the target referred to in the text.
To gain deeper insights into RESMatch, we conducted comprehensive visualizations, as depicted in Fig. \ref{fig:vis1}. In Fig. \ref{fig:vis1} (a), it is evident that RESMatch's predictions excel in various aspects. Examples like Exp-1 and Exp-2 showcase more accurate target localization, while Exp-3 and Exp-4 highlight improved target recognition. Additionally, examples like Exp-5 and Exp-6 demonstrate RESMatch's proficiency in precise boundary contour recognition.

In Fig. \ref{fig:vis1} (b), we further compare pseudo-labels with and without TA and MAG. These visualizations clearly illustrate that the incorporation of both designs significantly enhances the quality of pseudo-labels.

% While RESMatch demonstrates remarkable performance, there are instances owomanon the rightf failure, as visualized in Fig. \ref{fig:vis2}. Notably, challenges arise in handling highly abstract expressions, as observed in Exp-13 and Exp-14, where multiple directional terms within the expression pose difficulties. Failures also occur in instances like Exp-15 and Exp-16, where ambiguity in the text due to spelling errors and incomplete expressions leads to challenges. Moreover, ambiguity in the image contributes to failures, as seen in Exp-17 and Exp-18, making it challenging to precisely distinguish the target referred to in the text.

RESMatch excels in performance but faces challenges, as depicted in Fig. \ref{fig:vis2}. Handling highly abstract expressions, as in Exp-13 and Exp-14, with multiple directional terms, poses difficulties. Failures, evident in Exp-15 and Exp-16, result from text ambiguity due to spelling errors and incomplete expressions. Additionally, ambiguity in the image, as observed in Exp-17 and Exp-18, complicates the precise identification of the target mentioned in the text. 


% \begin{figure}[h]
%   \centering
%   \captionsetup[subfigure]{labelformat=empty} % 隐藏子图标签 (a), (b), ...
% \subfloat[]{
%     \setlength{\tabcolsep}{1.2mm}{
%     \begin{tabular}{ccc}
%   \multicolumn{1}{c}{Input}  & \multicolumn{1}{c}{GT} & \multicolumn{1}{c}{RESMatch} \\
%   \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp13-1.png} &
%   \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp13-3.png} &
%   \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp13-2.png} \\
%     \multicolumn{3}{c}{\makebox[0pt]{\centering Exp-13: left half of right \\ sandwich}} \\
 
%   \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp15-1.png} &
%   \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp15-3.png} &
%   \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp15-2.png} \\
%     \multicolumn{3}{c}{\makebox[0pt]{\centering Exp-15: cather}} \\

% \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp17-1.png} &
%   \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp17-3.png} &
%   \includegraphics[scale=0.119]{author-kit-CVPR2024-v2/sec/expfig/exp17-2.png} \\
%     \multicolumn{3}{c}{\makebox[0pt]{\centering Exp-17: the mans hair on right}} \\
% \end{tabular}}

%   }

  
%   \vspace{-15pt} % 根据需要调整垂直间距
%     \caption{\textbf{False cases in RESMatch.} It demonstrates that RESMatch still fails in some hard examples. Such as abstract expressions and the ambiguity of text or images.}
%   \label{fig:vis2}
% \end{figure}



==> author-kit-CVPR2024-v2/5_conclusion.tex <==


\section{Conclusion}
This work presented RESMatch, the first semi-supervised learning (SSL) approach specifically tailored for referring expression segmentation (RES). RESMatch confronts the complex challenges inherent to RES by integrating three key design adaptations: a revised approach to strong perturbation, the application of text augmentation, and the introduction of quality adjustments for pseudo-labels and strong-weak supervision. Extensive evaluation across multiple RES datasets confirms the superior performance of RESMatch over existing SSL methods, underscoring its effectiveness in reducing reliance on extensive data annotation, a key challenge in RES. The promising results not only establish RESMatch as a new solution for RES but also open up new avenues for future research in semi-supervised learning for RES and potentially other tasks involving complex language-vision interactions. 


==> author-kit-CVPR2024-v2/preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


